Three Cars Approaching within 100m! Enhancing Distant Geometry by Tri-Axis Voxel Scanning for Camera-based Semantic Scene Completion

Camera-based Semantic Scene Completion (SSC) is gaining attentions in the 3D perception field. However, properties such as perspective and occlusion lead to the underestimation of the geometry in distant regions, posing a critical issue for safety-focused autonomous driving systems. To tackle this, we propose ScanSSC, a novel camera-based SSC model composed of a Scan Module and Scan Loss, both designed to enhance distant scenes by leveraging context from near-viewpoint scenes. The Scan Module uses axis-wise masked attention, where each axis employing a near-to-far cascade masking that enables distant voxels to capture relationships with preceding voxels. In addition, the Scan Loss computes the cross-entropy along each axis between cumulative logits and corresponding class distributions in a near-to-far direction, thereby propagating rich context-aware signals to distant voxels. Leveraging the synergy between these components, ScanSSC achieves state-of-the-art performance, with IoUs of 44.54 and 48.29, and mIoUs of 17.40 and 20.14 on the SemanticKITTI and SSCBench-KITTI-360 benchmarks.

==> figure/fig.A.3_Loss.tex <==
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.32\linewidth}
        \subfloat[Depth-axis]{\includegraphics[width=\linewidth]{figure/Training_mIoU.pdf}}
        \label{fig:training_miou}
    \end{subfigure}
    \hspace{0.00\linewidth}
    \begin{subfigure}{0.32\linewidth}
        \subfloat[Width-axis]{\includegraphics[width=\linewidth]{figure/Sem_Scal_Loss.pdf}}
        \label{fig:sem_scal_loss}
    \end{subfigure}
    \hspace{0.00\linewidth}
    \begin{subfigure}{0.32\linewidth}
        \subfloat[Height-axis]{\includegraphics[width=\linewidth]{figure/Geo_Scal_Loss.pdf}}
        \label{fig:geo_scal_loss}
    \end{subfigure}
    
% \vspace{-.2cm}
    \caption{
    }
    \label{fig:appendix_loss}
\end{figure}
% \vspace{-0.6cm}

==> table/ablation_ScanLoss.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[h]
\centering
{%
\begin{tabular}{l|cc}
\hline
\rowcolor[HTML]{FFFFFF} 
Method & IoU                                               & mIoU  \\ \hline
\rowcolor[HTML]{FFFFFF} 
(a) $\mathcal{L}_{ce}+\mathcal{L}_{ce}^{dep}+\mathcal{L}_{ce}^{wid}+\mathcal{L}_{ce}^{hgt}$     & 46.08                                             & 16.25 \\
\rowcolor[HTML]{FFFFFF} 
(b) $\mathcal{L}^{tri}_{ce}$     & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}\textbf{46.15}} & 16.50 \\
\hline
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}(c) ScanSSC ($\mathcal{L}_{ce}+\mathcal{L}_{scan}$) & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}45.95} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}\textbf{17.12}} \\ \hline
\end{tabular}%
}
\caption{Ablation of Scan Loss}
\label{tab:ablation_ScanLoss}
\end{table}

==> table/ablation_loss_scale.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[h]
\centering
\setlength\tabcolsep{15pt}\resizebox{.6\linewidth}{!}{%
\begin{tabular}{c|cc}
\hline
   \multicolumn{1}{c|}{$\lambda_{scan}$}  &     IoU  & mIoU      \\
   \hline
   0.1 & 46.87 & 16.56 \\
   0.5 & 45.75 & 16.52 \\
   0.8 & 45.7 & 16.79 \\
   1. & 45.95 &\textbf{17.12} \\
   1.2 & 45.66 & 16.63 \\
   2. & 45.43 & 16.88 \\
   5. & 45.62 & 16.75 \\
   10. & 45.05 & 16.72 \\
\hline
\end{tabular}%
}
\caption{Performance Comparison by Loss Scaling Coefficient for Scan Loss.}
\label{tab:ablation_lossscale}
% \vspace{-.2cm}
\end{table}

==> table/ablation_mask_ratio.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\centering
\setlength\tabcolsep{12pt}\resizebox{\columnwidth}{!}{%
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c }
\hline
 &
   &
  \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}Depth} &
  \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}Width} &
  \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}Height} \\ \cline{3-8} 
 &
   &
  IoU &
  mIoU &
  IoU &
  mIoU &
  IoU &
  mIoU \\ \hline
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}} &
  0\% &
   45.58&
   16.21&
  46.07&
   16.42&
  \cellcolor[HTML]{EFEFEF}45.95 &
  \cellcolor[HTML]{EFEFEF}\textbf{17.12} \\
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}} &
  25\% &
   45.90 &
   16.57 &
   45.98&
   16.64&
   46.27 &
   16.77
   \\
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}} &
  50\% &
  \cellcolor[HTML]{EFEFEF}45.95 &
  \cellcolor[HTML]{EFEFEF}\textbf{17.12} &
  \cellcolor[HTML]{EFEFEF}45.95 &
  \cellcolor[HTML]{EFEFEF}\textbf{17.12} &
   45.98 &
   16.69
   \\
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}} &
  75\% &
   46.86&
   16.82&
   45.95&
   16.64&
   46.53 &
   16.53
   \\
\multicolumn{1}{c|}{\multirow{-5}{*}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}c@{}}margin\\ region\\ ratio\end{tabular}}} &
  100\% & 45.83
   &{16.73}
   &46.02
   &{16.52}
   &46.12
   &{16.52}
   \\ \hline
\end{tabular}%
}
\caption{Ablation of margin region ratio of masks in the Scan Module. The gray-colored cell represents the default setting.}
% The gray-colored cell represents the default configuration, while the bolded and underlined results indicate the best and second-best scores, respectively.
\label{tab:ablation_mask_ratio}
% \vspace{-0.6cm}
\end{table}
% \vspace{-0.4cm}

==> table/rebuttal_IoUs.tex <==
\newcommand{\colorboxlabel}[2]{\raisebox{0pt}[0pt][0pt]{\tikz{\node[fill=#1, minimum width=0.28cm, minimum height=0.28cm, inner sep=0pt] {};}}~#2}
\newcommand{\rotatebigtext}[1]{\rotatebox{90}{\fontsize{8}{8}\selectfont #1}}
\newcommand{\rotatetinytext}[1]{\rotatebox{90}{\fontsize{4}{4}\selectfont #1}}
\newcommand{\rotateemptytext}[1]{\rotatebox{90}{\fontsize{2}{2}\selectfont #1}}
\newcommand{\rotatabovetext}[1]{\rotatebox{90}{\fontsize{5}{5}\selectfont #1}}
\definecolor{custom_road}{RGB}{255, 0, 255}
\definecolor{custom_sidewalk}{RGB}{75, 0, 75}
\definecolor{custom_parking}{RGB}{255, 150, 255}
\definecolor{custom_other_ground}{RGB}{175, 0, 75}
\definecolor{custom_building}{RGB}{255, 200, 0}
\definecolor{custom_car}{RGB}{100, 150, 245}
\definecolor{custom_truck}{RGB}{80, 30, 180}
\definecolor{custom_bicycle}{RGB}{100, 230, 245}
\definecolor{custom_motorcycle}{RGB}{30, 60, 150}
\definecolor{custom_other_veh}{RGB}{0, 0, 255}
\definecolor{custom_vegetation}{RGB}{0, 175, 0}
\definecolor{custom_trunk}{RGB}{135, 60, 0}
\definecolor{custom_terrain}{RGB}{150, 240, 80}
\definecolor{custom_person}{RGB}{255, 30, 30}
\definecolor{custom_bicyclist}{RGB}{255, 40, 20}
\definecolor{custom_motorcyclist}{RGB}{150, 30, 90}
\definecolor{custom_fence}{RGB}{255, 120, 50}
\definecolor{custom_pole}{RGB}{255, 240, 150}
\definecolor{custom_traf_sign}{RGB}{255, 0, 0}
\begin{table}[hbt!]
\centering
% \resizebox{\textwidth}{!}{
\vspace{-.2cm}
\setlength\tabcolsep{3pt}\resizebox{\linewidth}{!}{
\begin{tabular}{l|clclclclclclclclclclclclclclclclclclcl}
\hline
 &
  % \multicolumn{1}{l}{} &
  %  &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} \\
 % &
 %  \multicolumn{1}{l}{} &
   &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{road} \newline \textcolor{white}{\rotatetinytext{1}} \newline \rotatetinytext{(15.30\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{sidewalk} \newline \textcolor{white}{\rotatetinytext{1}} \newline \rotatetinytext{(11.13\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{parking} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(1.12\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{other-grnd.} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.56\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{building} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(14.1\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{car} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(3.92\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{truck} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.16\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{bicycle} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.03\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{motorcycle} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.03\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{other-veh.} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.20\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{vegetation} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(39.3\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{trunk} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.51\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{terrain} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(9.17\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{person} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.07\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{bicyclist} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.07\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{motorcyclist} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.05\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{fence} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(3.90\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{pole} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.29\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{traf.-sign} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.08\%)}} \\
Method &
  % IoU &
  % \multicolumn{1}{c|}{mIoU} &
  \multicolumn{2}{c}{\colorboxlabel{custom_road}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_sidewalk}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_parking}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_other_ground}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_building}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_car}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_truck}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_bicycle}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_motorcycle}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_other_veh}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_vegetation}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_trunk}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_terrain}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_person}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_bicyclist}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_motorcyclist}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_fence}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_pole}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_traf_sign}{}} \\ \hline


  \multicolumn{39}{c}{Depth-Axis}\\\hline
  
 % \multicolumn{1}{l|}{VoxFormer}&
 % % \textbf{{44.54}} &
 % %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 %  \multicolumn{2}{c}{\textbf{{66.20}}} &
 %  \multicolumn{2}{c}{\textbf{{35.90}}} &
 %  \multicolumn{2}{c}{\textbf{{35.10}}} &
 %  \multicolumn{2}{c}{\textbf{{12.50}}} &
 %  \multicolumn{2}{c}{25.30} &
 %  \multicolumn{2}{c}{\underline{{27.10}}} &
 %  \multicolumn{2}{c}{3.50} &
 %  \multicolumn{2}{c}{3.50} &
 %  \multicolumn{2}{c}{\textbf{{3.20}}} &
 %  \multicolumn{2}{c}{\underline{{6.10}}} &
 %  \multicolumn{2}{c}{\underline{{25.20}}} &
 %  \multicolumn{2}{c}{\underline{{11.00}}} &
 %  \multicolumn{2}{c}{\underline{{30.60}}} &
 %  \multicolumn{2}{c}{1.80} &
 %  \multicolumn{2}{c}{\textbf{{5.30}}} &
 %  \multicolumn{2}{c}{0.70} &
 %  \multicolumn{2}{c}{\underline{{20.50}}} &
 %  \multicolumn{2}{c}{8.40} &
 %  \multicolumn{2}{c}{\underline{{8.90}}} \\ 

  
 % \multicolumn{1}{l|}{CGFormer}&
 % % \textbf{{44.54}} &
 % %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 % % 38.69 / 11.60 4gpu
 %  \multicolumn{2}{c}{{{54.69}}} &
 %  \multicolumn{2}{c}{{{24.69}}} &
 %  \multicolumn{2}{c}{{{20.17}}} &
 %  \multicolumn{2}{c}{{{\textbf{0.04}}}} &
 %  \multicolumn{2}{c}{17.70} &
 %  \multicolumn{2}{c}{\textbf{{21.01}}} &
 %  \multicolumn{2}{c}{\textbf{13.85}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{{{0.00}}} &
 %  \multicolumn{2}{c}{{{0.78}}} &
 %  \multicolumn{2}{c}{{{21.95}}} &
 %  \multicolumn{2}{c}{\textbf{{2.74}}} &
 %  \multicolumn{2}{c}{\textbf{{34.02}}} &
 %  \multicolumn{2}{c}{\textbf{0.15}} &
 %  \multicolumn{2}{c}{{{0.05}}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{{{5.45}}} &
 %  \multicolumn{2}{c}{\textbf{1.22}} &
 %  \multicolumn{2}{c}{\textbf{{1.98}}} \\ 

  
 \multicolumn{1}{l|}{CGFormer}&
 % \textbf{{44.54}} &
 %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 % 38.66 / 11.54 7gpu
  \multicolumn{2}{c}{{{54.73}}} &
  \multicolumn{2}{c}{{{24.69}}} &
  \multicolumn{2}{c}{{{20.02}}} &
  \multicolumn{2}{c}{{{\textbf{0.05}}}} &
  \multicolumn{2}{c}{17.66} &
  \multicolumn{2}{c}{\textbf{{21.10}}} &
  \multicolumn{2}{c}{\textbf{12.55}} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{{{0.00}}} &
  \multicolumn{2}{c}{{{0.97}}} &
  \multicolumn{2}{c}{{{21.94}}} &
  \multicolumn{2}{c}{\textbf{{2.74}}} &
  \multicolumn{2}{c}{\textbf{{34.03}}} &
  \multicolumn{2}{c}{\textbf{0.14}} &
  \multicolumn{2}{c}{{{0.08}}} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{{{5.46}}} &
  \multicolumn{2}{c}{\textbf{1.23}} &
  \multicolumn{2}{c}{\textbf{{1.89}}} \\ 

 % \multicolumn{1}{l|}{CGFormer}&
 % % \textbf{{44.54}} &
 % %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 % % 38.67 / 11.93
 %  \multicolumn{2}{c}{{{54.64}}} &
 %  \multicolumn{2}{c}{{{24.67}}} &
 %  \multicolumn{2}{c}{{{20.42}}} &
 %  \multicolumn{2}{c}{{{0.05}}} &
 %  \multicolumn{2}{c}{17.66} &
 %  \multicolumn{2}{c}{\textbf{{21.07}}} &
 %  \multicolumn{2}{c}{\textbf{19.90}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{{{0.00}}} &
 %  \multicolumn{2}{c}{{{0.92}}} &
 %  \multicolumn{2}{c}{{{21.95}}} &
 %  \multicolumn{2}{c}{\textbf{{2.71}}} &
 %  \multicolumn{2}{c}{\textbf{{33.91}}} &
 %  \multicolumn{2}{c}{\textbf{0.11}} &
 %  \multicolumn{2}{c}{{{0.07}}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{{{5.45}}} &
 %  \multicolumn{2}{c}{\textbf{1.22}} &
 %  \multicolumn{2}{c}{\textbf{{1.95}}} \\ 
  
 % \multicolumn{1}{l|}{\textbf{ScanSSC }}&
 % % \textbf{{44.54}} &
 % %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 % % 38.69 / 11.80
 %  \multicolumn{2}{c}{\textbf{{55.69}}} &
 %  \multicolumn{2}{c}{\textbf{{25.82}}} &
 %  \multicolumn{2}{c}{\textbf{{23.55}}} &
 %  \multicolumn{2}{c}{{{0.00}}} &
 %  \multicolumn{2}{c}{\textbf{18.01}} &
 %  \multicolumn{2}{c}{{{20.15}}} &
 %  \multicolumn{2}{c}{7.49} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{{{0.00}}} &
 %  \multicolumn{2}{c}{\textbf{{3.16}}} &
 %  \multicolumn{2}{c}{\textbf{{23.34}}} &
 %  \multicolumn{2}{c}{{{2.21}}} &
 %  \multicolumn{2}{c}{{{32.61}}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{\textbf{{0.57}}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{\textbf{{6.68}}} &
 %  \multicolumn{2}{c}{1.07} &
 %  \multicolumn{2}{c}{{{1.76}}} \\ \hline

  
 % \multicolumn{1}{l|}{\textbf{ScanSSC }}&
 % % \textbf{{44.54}} &
 % %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 % % 38.69 / 11.80
 %  \multicolumn{2}{c}{\textbf{{55.65}}} &
 %  \multicolumn{2}{c}{\textbf{{25.79}}} &
 %  \multicolumn{2}{c}{\textbf{{23.66}}} &
 %  \multicolumn{2}{c}{{{0.00}}} &
 %  \multicolumn{2}{c}{\textbf{17.96}} &
 %  \multicolumn{2}{c}{{{20.21}}} &
 %  \multicolumn{2}{c}{9.50} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{{{0.00}}} &
 %  \multicolumn{2}{c}{\textbf{{3.31}}} &
 %  \multicolumn{2}{c}{\textbf{{23.33}}} &
 %  \multicolumn{2}{c}{{{2.18}}} &
 %  \multicolumn{2}{c}{{{32.54}}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{\textbf{{0.59}}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{\textbf{{6.69}}} &
 %  \multicolumn{2}{c}{1.07} &
 %  \multicolumn{2}{c}{{{1.77}}} \\ \hline
  
 \multicolumn{1}{l|}{\textbf{ScanSSC }}&
 % \textbf{{44.54}} &
 %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 % 5gpu 38.66 / 11.89
  \multicolumn{2}{c}{\textbf{{55.67}}} &
  \multicolumn{2}{c}{\textbf{{25.82}}} &
  \multicolumn{2}{c}{\textbf{{23.68}}} &
  \multicolumn{2}{c}{{{0.00}}} &
  \multicolumn{2}{c}{\textbf{17.89}} &
  \multicolumn{2}{c}{{{20.21}}} &
  \multicolumn{2}{c}{12.20} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{{{0.00}}} &
  \multicolumn{2}{c}{\textbf{{2.72}}} &
  \multicolumn{2}{c}{\textbf{{23.34}}} &
  \multicolumn{2}{c}{{{2.19}}} &
  \multicolumn{2}{c}{{{32.17}}} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{\textbf{{0.57}}} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{\textbf{{6.76}}} &
  \multicolumn{2}{c}{1.05} &
  \multicolumn{2}{c}{{{1.75}}} \\ \hline
  
  \multicolumn{39}{c}{Width-Axis}\\\hline
  
 % \multicolumn{1}{l|}{VoxFormer}&
 % % \textbf{{44.54}} &
 % %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 %  \multicolumn{2}{c}{\textbf{{66.20}}} &
 %  \multicolumn{2}{c}{\textbf{{35.90}}} &
 %  \multicolumn{2}{c}{\textbf{{35.10}}} &
 %  \multicolumn{2}{c}{\textbf{{12.50}}} &
 %  \multicolumn{2}{c}{25.30} &
 %  \multicolumn{2}{c}{\underline{{27.10}}} &
 %  \multicolumn{2}{c}{3.50} &
 %  \multicolumn{2}{c}{3.50} &
 %  \multicolumn{2}{c}{\textbf{{3.20}}} &
 %  \multicolumn{2}{c}{\underline{{6.10}}} &
 %  \multicolumn{2}{c}{\underline{{25.20}}} &
 %  \multicolumn{2}{c}{\underline{{11.00}}} &
 %  \multicolumn{2}{c}{\underline{{30.60}}} &
 %  \multicolumn{2}{c}{1.80} &
 %  \multicolumn{2}{c}{\textbf{{5.30}}} &
 %  \multicolumn{2}{c}{0.70} &
 %  \multicolumn{2}{c}{\underline{{20.50}}} &
 %  \multicolumn{2}{c}{8.40} &
 %  \multicolumn{2}{c}{\underline{{8.90}}} \\ 

 % \multicolumn{1}{l|}{CGFormer}&
 % % \textbf{{44.54}} &
 % %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 % % 22.06 / 5.05 4gpu
 %  \multicolumn{2}{c}{{{28.40}}} &
 %  \multicolumn{2}{c}{{{10.78}}} &
 %  \multicolumn{2}{c}{{{5.00}}} &
 %  \multicolumn{2}{c}{{{\textbf{0.30}}}} &
 %  \multicolumn{2}{c}{\textbf{8.26}} &
 %  \multicolumn{2}{c}{{{3.42}}} &
 %  \multicolumn{2}{c}{\textbf{1.67}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{{{0.00}}} &
 %  \multicolumn{2}{c}{{{0.00}}} &
 %  \multicolumn{2}{c}{{{8.28}}} &
 %  \multicolumn{2}{c}{\textbf{{0.87}}} &
 %  \multicolumn{2}{c}{\textbf{{26.97}}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{{{0.00}}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{{{1.61}}} &
 %  \multicolumn{2}{c}{0.23} &
 %  \multicolumn{2}{c}{{{0.20}}} \\ 
  
 % \multicolumn{1}{l|}{CGFormer}&
 % % \textbf{{44.54}} &
 % %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 % % 22.06 / 5.10
 %  \multicolumn{2}{c}{{{28.48}}} &
 %  \multicolumn{2}{c}{{{10.77}}} &
 %  \multicolumn{2}{c}{{{4.95}}} &
 %  \multicolumn{2}{c}{{{0.27}}} &
 %  \multicolumn{2}{c}{\textbf{8.26}} &
 %  \multicolumn{2}{c}{{{3.38}}} &
 %  \multicolumn{2}{c}{\textbf{2.66}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{{{0.00}}} &
 %  \multicolumn{2}{c}{{{0.00}}} &
 %  \multicolumn{2}{c}{{{8.32}}} &
 %  \multicolumn{2}{c}{\textbf{{0.89}}} &
 %  \multicolumn{2}{c}{\textbf{{26.92}}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{{{0.00}}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{{{1.58}}} &
 %  \multicolumn{2}{c}{0.20} &
 %  \multicolumn{2}{c}{{{0.25}}} \\ 

 % \multicolumn{1}{l|}{CGFormer}&
 % % \textbf{{44.54}} &
 % %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 % % 50
 %  \multicolumn{2}{c}{{{34.41}}} &
 %  \multicolumn{2}{c}{{{13.66}}} &
 %  \multicolumn{2}{c}{{{8.01}}} &
 %  \multicolumn{2}{c}{{{{0.31}}}} &
 %  \multicolumn{2}{c}{\textbf{15.84}} &
 %  \multicolumn{2}{c}{{{5.81}}} &
 %  \multicolumn{2}{c}{\textbf{0.67}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{{{0.00}}} &
 %  \multicolumn{2}{c}{{{\textbf{0.10}}}} &
 %  \multicolumn{2}{c}{{{12.75}}} &
 %  \multicolumn{2}{c}{\textbf{{3.07}}} &
 %  \multicolumn{2}{c}{\textbf{{33.76}}} &
 %  \multicolumn{2}{c}{0.19} &
 %  \multicolumn{2}{c}{{{0.31}}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{{{1.60}}} &
 %  \multicolumn{2}{c}{1.22} &
 %  \multicolumn{2}{c}{{{\textbf{1.59}}}} \\ 
  
 \multicolumn{1}{l|}{CGFormer}&
 % \textbf{{44.54}} &
 %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 % 50/ 7gpu
  \multicolumn{2}{c}{{{34.26}}} &
  \multicolumn{2}{c}{{{13.67}}} &
  \multicolumn{2}{c}{{{8.67}}} &
  \multicolumn{2}{c}{{{{0.30}}}} &
  \multicolumn{2}{c}{\textbf{15.81}} &
  \multicolumn{2}{c}{{{5.55}}} &
  \multicolumn{2}{c}{{0.51}} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{{{0.00}}} &
  \multicolumn{2}{c}{{{\textbf{0.13}}}} &
  \multicolumn{2}{c}{{{12.69}}} &
  \multicolumn{2}{c}{\textbf{{3.07}}} &
  \multicolumn{2}{c}{\textbf{{33.76}}} &
  \multicolumn{2}{c}{0.18} &
  \multicolumn{2}{c}{{{0.28}}} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{{{1.43}}} &
  \multicolumn{2}{c}{1.20} &
  \multicolumn{2}{c}{{{{1.41}}}} \\ 
  
 % \multicolumn{1}{l|}{\textbf{ScanSSC }}&
 % % \textbf{{44.54}} &
 % %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 % % 21.79 / 5.40
 %  \multicolumn{2}{c}{\textbf{{31.65}}} &
 %  \multicolumn{2}{c}{\textbf{{13.22}}} &
 %  \multicolumn{2}{c}{\textbf{{9.23}}} &
 %  \multicolumn{2}{c}{{{0.22}}} &
 %  \multicolumn{2}{c}{7.89} &
 %  \multicolumn{2}{c}{\textbf{{3.77}}} &
 %  \multicolumn{2}{c}{0.53} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{{{0.00}}} &
 %  \multicolumn{2}{c}{{{0.00}}} &
 %  \multicolumn{2}{c}{\textbf{{9.09}}} &
 %  \multicolumn{2}{c}{{{0.53}}} &
 %  \multicolumn{2}{c}{{{23.94}}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{{{0.00}}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{\textbf{{1.87}}} &
 %  \multicolumn{2}{c}{{\textbf{0.27}}} &
 %  \multicolumn{2}{c}{{{\textbf{0.34}}}} \\ \hline

 
 \multicolumn{1}{l|}{\textbf{ScanSSC }}&
 % \textbf{{44.54}} &
 %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 % 50/ 29.39 / 7.40
  \multicolumn{2}{c}{\textbf{{37.34}}} &
  \multicolumn{2}{c}{\textbf{{16.25}}} &
  \multicolumn{2}{c}{\textbf{{11.07}}} &
  \multicolumn{2}{c}{{{\textbf{0.36}}}} &
  \multicolumn{2}{c}{14.65} &
  \multicolumn{2}{c}{\textbf{{6.23}}} &
  \multicolumn{2}{c}{\textbf{0.66}} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{{{0.00}}} &
  \multicolumn{2}{c}{{{0.04}}} &
  \multicolumn{2}{c}{\textbf{{13.44}}} &
  \multicolumn{2}{c}{{{2.71}}} &
  \multicolumn{2}{c}{{{31.74}}} &
  \multicolumn{2}{c}{\textbf{0.25}} &
  \multicolumn{2}{c}{{{\textbf{1.47}}}} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{\textbf{{1.73}}} &
  \multicolumn{2}{c}{{\textbf{1.26}}} &
  \multicolumn{2}{c}{{{{\textbf{1.47}}}}} \\ \hline
  
 
 % \multicolumn{1}{l|}{\textbf{ScanSSC }}&
 % % \textbf{{44.54}} &
 % %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 % % 50/ 3gpu 29.39 / 7.42
 %  \multicolumn{2}{c}{\textbf{{37.34}}} &
 %  \multicolumn{2}{c}{\textbf{{16.25}}} &
 %  \multicolumn{2}{c}{\textbf{{11.07}}} &
 %  \multicolumn{2}{c}{{{\textbf{0.36}}}} &
 %  \multicolumn{2}{c}{14.65} &
 %  \multicolumn{2}{c}{\textbf{{6.23}}} &
 %  \multicolumn{2}{c}{\textbf{0.66}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{{{0.00}}} &
 %  \multicolumn{2}{c}{{{0.04}}} &
 %  \multicolumn{2}{c}{\textbf{{13.44}}} &
 %  \multicolumn{2}{c}{{{2.71}}} &
 %  \multicolumn{2}{c}{{{31.74}}} &
 %  \multicolumn{2}{c}{\textbf{0.25}} &
 %  \multicolumn{2}{c}{{{\textbf{1.47}}}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{\textbf{{1.73}}} &
 %  \multicolumn{2}{c}{{\textbf{1.26}}} &
 %  \multicolumn{2}{c}{{{{\textbf{1.47}}}}} \\ \hline
  \multicolumn{39}{c}{Height-Axis}\\\hline
  
 % \multicolumn{1}{l|}{VoxFormer}&
 % % \textbf{{44.54}} &
 % %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 %  \multicolumn{2}{c}{\textbf{{66.20}}} &
 %  \multicolumn{2}{c}{\textbf{{35.90}}} &
 %  \multicolumn{2}{c}{\textbf{{35.10}}} &
 %  \multicolumn{2}{c}{\textbf{{12.50}}} &
 %  \multicolumn{2}{c}{25.30} &
 %  \multicolumn{2}{c}{\underline{{27.10}}} &
 %  \multicolumn{2}{c}{3.50} &
 %  \multicolumn{2}{c}{3.50} &
 %  \multicolumn{2}{c}{\textbf{{3.20}}} &
 %  \multicolumn{2}{c}{\underline{{6.10}}} &
 %  \multicolumn{2}{c}{\underline{{25.20}}} &
 %  \multicolumn{2}{c}{\underline{{11.00}}} &
 %  \multicolumn{2}{c}{\underline{{30.60}}} &
 %  \multicolumn{2}{c}{1.80} &
 %  \multicolumn{2}{c}{\textbf{{5.30}}} &
 %  \multicolumn{2}{c}{0.70} &
 %  \multicolumn{2}{c}{\underline{{20.50}}} &
 %  \multicolumn{2}{c}{8.40} &
 %  \multicolumn{2}{c}{\underline{{8.90}}} \\ 

% \multicolumn{1}{l|}{CGFormer}&
%  % \textbf{{44.54}} &
%  %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
%  % 59.40 / 16.65
%   \multicolumn{2}{c}{{{66.01}}} &
%   \multicolumn{2}{c}{{{32.81}}} &
%   \multicolumn{2}{c}{{{20.84}}} &
%   \multicolumn{2}{c}{{{0.16}}} &
%   \multicolumn{2}{c}{\textbf{23.13}} &
%   \multicolumn{2}{c}{\textbf{{36.91}}} &
%   \multicolumn{2}{c}{13.39} &
%   \multicolumn{2}{c}{\textbf{5.23}} &
%   \multicolumn{2}{c}{\textbf{{3.44}}} &
%   \multicolumn{2}{c}{{{8.51}}} &
%   \multicolumn{2}{c}{{{27.41}}} &
%   \multicolumn{2}{c}{\textbf{{9.63}}} &
%   \multicolumn{2}{c}{\textbf{{40.14}}} &
%   \multicolumn{2}{c}{2.88} &
%   \multicolumn{2}{c}{{{5.67}}} &
%   \multicolumn{2}{c}{0.00} &
%   \multicolumn{2}{c}{{{9.06}}} &
%   \multicolumn{2}{c}{{\textbf{10.98}}} &
%   \multicolumn{2}{c}{{{\textbf{0.19}}}} \\ 
  
\multicolumn{1}{l|}{CGFormer}&
 % \textbf{{44.54}} &
 %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 % 7gpu 59.40 / 16.55
  \multicolumn{2}{c}{{{66.07}}} &
  \multicolumn{2}{c}{{{32.85}}} &
  \multicolumn{2}{c}{{{20.50}}} &
  \multicolumn{2}{c}{{{0.18}}} &
  \multicolumn{2}{c}{\textbf{23.15}} &
  \multicolumn{2}{c}{\textbf{{36.90}}} &
  \multicolumn{2}{c}{12.48} &
  \multicolumn{2}{c}{\textbf{5.10}} &
  \multicolumn{2}{c}{\textbf{{3.47}}} &
  \multicolumn{2}{c}{{{8.19}}} &
  \multicolumn{2}{c}{{{27.46}}} &
  \multicolumn{2}{c}{\textbf{{9.61}}} &
  \multicolumn{2}{c}{\textbf{{40.11}}} &
  \multicolumn{2}{c}{2.88} &
  \multicolumn{2}{c}{{{5.50}}} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{{{9.03}}} &
  \multicolumn{2}{c}{{\textbf{10.96}}} &
  \multicolumn{2}{c}{{{\textbf{0.19}}}} \\ 
  
 % \multicolumn{1}{l|}{CGFormer}&
 % % \textbf{{44.54}} &
 % %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 % % 59.39 / 16.80
 %  \multicolumn{2}{c}{{{66.00}}} &
 %  \multicolumn{2}{c}{{{32.81}}} &
 %  \multicolumn{2}{c}{{{20.84}}} &
 %  \multicolumn{2}{c}{{{0.17}}} &
 %  \multicolumn{2}{c}{\textbf{23.13}} &
 %  \multicolumn{2}{c}{\textbf{{36.90}}} &
 %  \multicolumn{2}{c}{\textbf{16.21}} &
 %  \multicolumn{2}{c}{\textbf{5.28}} &
 %  \multicolumn{2}{c}{\textbf{{3.56}}} &
 %  \multicolumn{2}{c}{{{8.54}}} &
 %  \multicolumn{2}{c}{{{27.43}}} &
 %  \multicolumn{2}{c}{\textbf{{9.62}}} &
 %  \multicolumn{2}{c}{\textbf{{40.07}}} &
 %  \multicolumn{2}{c}{2.89} &
 %  \multicolumn{2}{c}{{{5.62}}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{{{9.08}}} &
 %  \multicolumn{2}{c}{{10.98}} &
 %  \multicolumn{2}{c}{{{0.20}}} \\ 
  
 % \multicolumn{1}{l|}{\textbf{ScanSSC }}&
 % % \textbf{{44.54}} &
 % %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 % % 59.79 / 17.14
 %  \multicolumn{2}{c}{\textbf{{67.19}}} &
 %  \multicolumn{2}{c}{\textbf{{34.37}}} &
 %  \multicolumn{2}{c}{\textbf{{24.96}}} &
 %  \multicolumn{2}{c}{{{\textbf{0.20}}}} &
 %  \multicolumn{2}{c}{21.51} &
 %  \multicolumn{2}{c}{{{36.44}}} &
 %  \multicolumn{2}{c}{\textbf{13.40}} &
 %  \multicolumn{2}{c}{4.29} &
 %  \multicolumn{2}{c}{{{2.92}}} &
 %  \multicolumn{2}{c}{\textbf{{11.11}}} &
 %  \multicolumn{2}{c}{\textbf{{28.55}}} &
 %  \multicolumn{2}{c}{{{9.21}}} &
 %  \multicolumn{2}{c}{{{39.93}}} &
 %  \multicolumn{2}{c}{\textbf{3.44}} &
 %  \multicolumn{2}{c}{\textbf{{6.91}}} &
 %  \multicolumn{2}{c}{0.00} &
 %  \multicolumn{2}{c}{\textbf{{10.31}}} &
 %  \multicolumn{2}{c}{10.92} &
 %  \multicolumn{2}{c}{{{0.10}}} \\ \hline

    
 \multicolumn{1}{l|}{\textbf{ScanSSC }}&
 % \textbf{{44.54}} &
 %  \multicolumn{1}{c|}{\textbf{{17.40}}} &
 % 2gpu 59.78 / 17.18
  \multicolumn{2}{c}{\textbf{{67.21}}} &
  \multicolumn{2}{c}{\textbf{{34.39}}} &
  \multicolumn{2}{c}{\textbf{{24.96}}} &
  \multicolumn{2}{c}{{{\textbf{0.21}}}} &
  \multicolumn{2}{c}{21.50} &
  \multicolumn{2}{c}{{{36.45}}} &
  \multicolumn{2}{c}{\textbf{14.03}} &
  \multicolumn{2}{c}{4.29} &
  \multicolumn{2}{c}{{{2.94}}} &
  \multicolumn{2}{c}{\textbf{{11.20}}} &
  \multicolumn{2}{c}{\textbf{{28.54}}} &
  \multicolumn{2}{c}{{{9.23}}} &
  \multicolumn{2}{c}{{{39.96}}} &
  \multicolumn{2}{c}{\textbf{3.44}} &
  \multicolumn{2}{c}{\textbf{{6.89}}} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{\textbf{{10.30}}} &
  \multicolumn{2}{c}{10.92} &
  \multicolumn{2}{c}{{{0.10}}} \\ \hline
\end{tabular}}%
\vspace{-\baselineskip}
\caption{Quantitative results on SemanticKITTI val. set.}
\vspace{-.4cm}
\label{tab:rebuttal_iou}
\end{table}

==> table/rebuttal_attention.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[hbt!]
\centering
\vspace{-.3cm}
\setlength\tabcolsep{15pt}\resizebox{.7\linewidth}{!}{%
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c }
\hline
                          Method  & IoU   & mIoU  \\ \hline
(a) w.o. axis-specific mask                    & 46.01 & 16.64 \\ \hline
(b) w.o. spatial mixing network                    & 45.08 & 16.11 \\
(c) w.o. tri-feature fusion                    & 45.90 & 16.32 \\
(d) w.o. both                    & 44.91 & 15.90 \\\hline
% (d) w.o. both                    & 44.94 & 15.74 \\\hline
(e) $\mathcal{L}_{ce}^{tri}$                    & 46.08 & 16.25\\ 
(f) $\mathcal{L}_{ce}$ + $\mathcal{L}_{ce}^{dep}$ + $\mathcal{L}_{ce}^{wid}$ + $\mathcal{L}_{ce}^{hgt}$                    & 46.15 & 16.50\\ \hline
(g) ScanSSC (${L}_{ce}$ + $\mathcal{L}_{scan}$)                      & 45.95 & \textbf{17.12} \\ \hline
\end{tabular}}
% \vspace{-\baselineskip}
% \caption{Additional ablation studies on SemanticKITTI val. set.}
\vspace{-.5cm}
\label{tab:rebuttal_attention}
\end{table}

==> table/rebuttal_loss.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[hbt!]
\centering
\vspace{-.3cm}
\setlength\tabcolsep{20pt}\resizebox{.7\linewidth}{!}{%
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c }
\hline
                          Method  & IoU   & mIoU  \\ \hline
(a) $\mathcal{L}_{ce}^{tri}$                    & 46.08 & 16.25\\ 
(b) $\mathcal{L}_{ce}$ + $\mathcal{L}_{ce}^{dep}$ + $\mathcal{L}_{ce}^{wid}$ + $\mathcal{L}_{ce}^{hgt}$                    & 46.15 & 16.50\\ 
(c) $\mathcal{L}_{ce}$ + $\mathcal{L}_{scan}$ (ours)                     & 45.95 & \textbf{17.12} \\ \hline
\end{tabular}}
\vspace{-\baselineskip}
\caption{Ablation study of Scan Loss on SemanticKITTI val. set.}
\vspace{-.5cm}
\label{tab:rebuttal_loss}
\end{table}

==> table/results_SemanticKITTI_valid.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\newcommand{\colorboxlabel}[2]{\raisebox{0pt}[0pt][0pt]{\tikz{\node[fill=#1, minimum width=0.28cm, minimum height=0.28cm, inner sep=0pt] {};}}~#2}
\newcommand{\rotatebigtext}[1]{\rotatebox{90}{\fontsize{8}{8}\selectfont #1}}
\newcommand{\rotatetinytext}[1]{\rotatebox{90}{\fontsize{4}{4}\selectfont #1}}
\newcommand{\rotateemptytext}[1]{\rotatebox{90}{\fontsize{2}{2}\selectfont #1}}
\newcommand{\rotatabovetext}[1]{\rotatebox{90}{\fontsize{5}{5}\selectfont #1}}

\definecolor{custom_road}{RGB}{255, 0, 255}
\definecolor{custom_sidewalk}{RGB}{75, 0, 75}
\definecolor{custom_parking}{RGB}{255, 150, 255}
\definecolor{custom_other_ground}{RGB}{175, 0, 75}
\definecolor{custom_building}{RGB}{255, 200, 0}
\definecolor{custom_car}{RGB}{100, 150, 245}
\definecolor{custom_truck}{RGB}{80, 30, 180}
\definecolor{custom_bicycle}{RGB}{100, 230, 245}
\definecolor{custom_motorcycle}{RGB}{30, 60, 150}
\definecolor{custom_other_veh}{RGB}{0, 0, 255}
\definecolor{custom_vegetation}{RGB}{0, 175, 0}
\definecolor{custom_trunk}{RGB}{135, 60, 0}
\definecolor{custom_terrain}{RGB}{150, 240, 80}
\definecolor{custom_person}{RGB}{255, 30, 30}
\definecolor{custom_bicyclist}{RGB}{255, 40, 20}
\definecolor{custom_motorcyclist}{RGB}{150, 30, 90}
\definecolor{custom_fence}{RGB}{255, 120, 50}
\definecolor{custom_pole}{RGB}{255, 240, 150}
\definecolor{custom_traf_sign}{RGB}{255, 0, 0}


\begin{table*}[hbt!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccl|clclclclclclclclclclclclclclclclclclcl}
\hline
 &
&
  \multicolumn{1}{l}{} &
   &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} &
  \multicolumn{2}{l}{} \\
 &
 &
  \multicolumn{1}{l}{} &
   &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{road} \newline \textcolor{white}{\rotatetinytext{1}} \newline \rotatetinytext{(15.30\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{sidewalk} \newline \textcolor{white}{\rotatetinytext{1}} \newline \rotatetinytext{(11.13\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{parking} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(1.12\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{other-grnd.} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.56\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{building} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(14.1\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{car} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(3.92\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{truck} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.16\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{bicycle} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.03\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{motorcycle} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.03\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{other-veh.} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.20\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{vegetation} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(39.3\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{trunk} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.51\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{terrain} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(9.17\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{person} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.07\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{bicyclist} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.07\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{motorcyclist} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.05\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{fence} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(3.90\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{pole} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.29\%)}} &
  \multicolumn{2}{l}{\textcolor{white}{\rotatabovetext{1}} \newline \rotatebigtext{traf.-sign} \newline \textcolor{white}{\rotatetinytext{1}}\newline \rotatetinytext{(0.08\%)}} \\
Method &
Input&
  IoU &
  \multicolumn{1}{c|}{mIoU} &
  \multicolumn{2}{c}{\colorboxlabel{custom_road}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_sidewalk}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_parking}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_other_ground}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_building}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_car}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_truck}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_bicycle}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_motorcycle}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_other_veh}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_vegetation}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_trunk}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_terrain}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_person}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_bicyclist}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_motorcyclist}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_fence}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_pole}{}} &
  \multicolumn{2}{c}{\colorboxlabel{custom_traf_sign}{}} \\ \hline




 \multicolumn{1}{l|}{MonoScene~\cite{cao2022monoscene}} &
 \multicolumn{1}{c|}{M}&
   36.86&
  \multicolumn{1}{c|}{11.08} &
  \multicolumn{2}{c}{56.52} &
  \multicolumn{2}{c}{26.72} &
  \multicolumn{2}{c}{14.27} &
  \multicolumn{2}{c}{0.46} &
  \multicolumn{2}{c}{14.09} &
  \multicolumn{2}{c}{23.26} &
  \multicolumn{2}{c}{6.98} &
  \multicolumn{2}{c}{0.61} &
  \multicolumn{2}{c}{0.45} &
  \multicolumn{2}{c}{1.48} &
  \multicolumn{2}{c}{17.89} &
  \multicolumn{2}{c}{2.81} &
  \multicolumn{2}{c}{29.64} &
  \multicolumn{2}{c}{1.86} &
  \multicolumn{2}{c}{1.20} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{5.84} &
  \multicolumn{2}{c}{4.14} &
  \multicolumn{2}{c}{2.25} \\
 \multicolumn{1}{l|}{TPVFormer~\cite{huang2023tri}} &
 \multicolumn{1}{c|}{M}&
  35.61 &
  \multicolumn{1}{c|}{11.36} &
  \multicolumn{2}{c}{56.50} &
  \multicolumn{2}{c}{25.87} &
  \multicolumn{2}{c}{20.60} &
  \multicolumn{2}{c}{0.85} &
  \multicolumn{2}{c}{13.88} &
  \multicolumn{2}{c}{23.81} &
  \multicolumn{2}{c}{8.08} &
  \multicolumn{2}{c}{0.36} &
  \multicolumn{2}{c}{0.05} &
  \multicolumn{2}{c}{4.35} &
  \multicolumn{2}{c}{16.92} &
  \multicolumn{2}{c}{2.26} &
  \multicolumn{2}{c}{30.38} &
  \multicolumn{2}{c}{0.51} &
  \multicolumn{2}{c}{0.89} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{5.94} &
  \multicolumn{2}{c}{3.14} &
  \multicolumn{2}{c}{1.52} \\
 % \multicolumn{1}{l|}{SurroundOcc~\cite{wei2023surroundocc}} &
 % \multicolumn{1}{c|}{M}&
 %   &
 %  \multicolumn{1}{c|}{11.86} &
 %  \multicolumn{2}{c}{56.90} &
 %  \multicolumn{2}{c}{28.30} &
 %  \multicolumn{2}{c}{30.20} &
 %  \multicolumn{2}{c}{6.80} &
 %  \multicolumn{2}{c}{15.20} &
 %  \multicolumn{2}{c}{20.60} &
 %  \multicolumn{2}{c}{1.40} &
 %  \multicolumn{2}{c}{1.60} &
 %  \multicolumn{2}{c}{1.20} &
 %  \multicolumn{2}{c}{4.40} &
 %  \multicolumn{2}{c}{14.90} &
 %  \multicolumn{2}{c}{3.40} &
 %  \multicolumn{2}{c}{19.30} &
 %  \multicolumn{2}{c}{1.40} &
 %  \multicolumn{2}{c}{2.00} &
 %  \multicolumn{2}{c}{0.10} &
 %  \multicolumn{2}{c}{11.30} &
 %  \multicolumn{2}{c}{3.90} &
 %  \multicolumn{2}{c}{2.40} \\
\multicolumn{1}{l|}{OccFormer~\cite{zhang2023occformer}} &
\multicolumn{1}{c|}{M}&
  36.50 &
  \multicolumn{1}{c|}{13.46} &
  \multicolumn{2}{c}{58.85} &
  \multicolumn{2}{c}{26.88} &
  \multicolumn{2}{c}{19.61} &
  \multicolumn{2}{c}{0.31} &
  \multicolumn{2}{c}{14.40} &
  \multicolumn{2}{c}{25.09} &
  \multicolumn{2}{c}{25.53} &
  \multicolumn{2}{c}{0.81} &
  \multicolumn{2}{c}{1.19} &
  \multicolumn{2}{c}{8.52} &
  \multicolumn{2}{c}{19.63} &
  \multicolumn{2}{c}{3.93} &
  \multicolumn{2}{c}{32.62} &
  \multicolumn{2}{c}{2.78} &
  \multicolumn{2}{c}{2.82} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{5.61} &
  \multicolumn{2}{c}{4.26} &
  \multicolumn{2}{c}{2.86} \\
\multicolumn{1}{l|}{IAMSSC~\cite{xiao2024instance}} &
\multicolumn{1}{c|}{M}&
  44.29 &
  \multicolumn{1}{c|}{12.45} &
  \multicolumn{2}{c}{54.55} &
  \multicolumn{2}{c}{25.85} &
  \multicolumn{2}{c}{16.02} &
  \multicolumn{2}{c}{0.70} &
  \multicolumn{2}{c}{17.38} &
  \multicolumn{2}{c}{26.26} &
  \multicolumn{2}{c}{8.74} &
  \multicolumn{2}{c}{0.60} &
  \multicolumn{2}{c}{0.15} &
  \multicolumn{2}{c}{5.06} &
  \multicolumn{2}{c}{24.63} &
  \multicolumn{2}{c}{4.95} &
  \multicolumn{2}{c}{30.13} &
  \multicolumn{2}{c}{1.32} &
  \multicolumn{2}{c}{3.46} &
  \multicolumn{2}{c}{0.01} &
  \multicolumn{2}{c}{6.86} &
  \multicolumn{2}{c}{6.35} &
  \multicolumn{2}{c}{3.56} \\
% \multicolumn{1}{l|}{VoxFormer-S~\cite{li2023voxformer}} &
% \multicolumn{1}{c|}{S}&
%   42.95 &
%   \multicolumn{1}{c|}{12.20} &
%   \multicolumn{2}{c}{53.90} &
%   \multicolumn{2}{c}{25.30} &
%   \multicolumn{2}{c}{21.10} &
%   \multicolumn{2}{c}{5.60} &
%   \multicolumn{2}{c}{19.80} &
%   \multicolumn{2}{c}{20.80} &
%   \multicolumn{2}{c}{3.50} &
%   \multicolumn{2}{c}{1.00} &
%   \multicolumn{2}{c}{0.70} &
%   \multicolumn{2}{c}{3.70} &
%   \multicolumn{2}{c}{22.40} &
%   \multicolumn{2}{c}{7.50} &
%   \multicolumn{2}{c}{21.30} &
%   \multicolumn{2}{c}{1.40} &
%   \multicolumn{2}{c}{2.60} &
%   \multicolumn{2}{c}{0.20} &
%   \multicolumn{2}{c}{11.10} &
%   \multicolumn{2}{c}{5.10} &
%   \multicolumn{2}{c}{4.90} \\
\multicolumn{1}{l|}{VoxFormer-T~\cite{li2023voxformer}} &
\multicolumn{1}{c|}{S-T}&
  44.15 &
  \multicolumn{1}{c|}{13.35} &
  \multicolumn{2}{c}{53.57} &
  \multicolumn{2}{c}{26.32} &
  \multicolumn{2}{c}{19.69} &
  \multicolumn{2}{c}{0.42} &
  \multicolumn{2}{c}{19.54} &
  \multicolumn{2}{c}{26.54} &
  \multicolumn{2}{c}{7.26} &
  \multicolumn{2}{c}{1.28} &
  \multicolumn{2}{c}{0.56} &
  \multicolumn{2}{c}{7.81} &
  \multicolumn{2}{c}{26.10} &
  \multicolumn{2}{c}{6.10} &
  \multicolumn{2}{c}{33.06} &
  \multicolumn{2}{c}{1.93} &
  \multicolumn{2}{c}{1.97} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{7.31} &
  \multicolumn{2}{c}{9.15} &
  \multicolumn{2}{c}{4.94} \\
 % \multicolumn{1}{l|}{HASSC-S~\cite{wang2024not}} &
 % \multicolumn{1}{c|}{S}&
 %  43.40 &
 %  \multicolumn{1}{c|}{13.34} &
 %  \multicolumn{2}{c}{54.60} &
 %  \multicolumn{2}{c}{27.70} &
 %  \multicolumn{2}{c}{23.80} &
 %  \multicolumn{2}{c}{6.20} &
 %  \multicolumn{2}{c}{21.10} &
 %  \multicolumn{2}{c}{22.80} &
 %  \multicolumn{2}{c}{4.70} &
 %  \multicolumn{2}{c}{1.60} &
 %  \multicolumn{2}{c}{1.00} &
 %  \multicolumn{2}{c}{3.90} &
 %  \multicolumn{2}{c}{23.80} &
 %  \multicolumn{2}{c}{8.50} &
 %  \multicolumn{2}{c}{23.30} &
 %  \multicolumn{2}{c}{1.60} &
 %  \multicolumn{2}{c}{4.00} &
 %  \multicolumn{2}{c}{0.30} &
 %  \multicolumn{2}{c}{13.10} &
 %  \multicolumn{2}{c}{5.80} &
 %  \multicolumn{2}{c}{5.50} \\
 \multicolumn{1}{l|}{HASSC-T~\cite{wang2024not}} &
 \multicolumn{1}{c|}{S-T}&
  44.58 &
  \multicolumn{1}{c|}{14.74} &
  \multicolumn{2}{c}{57.23} &
  \multicolumn{2}{c}{29.08} &
  \multicolumn{2}{c}{19.89} &
  \multicolumn{2}{c}{\textbf{1.26}} &
  \multicolumn{2}{c}{20.19} &
  \multicolumn{2}{c}{27.33} &
  \multicolumn{2}{c}{17.06} &
  \multicolumn{2}{c}{1.07} &
  \multicolumn{2}{c}{1.14} &
  \multicolumn{2}{c}{8.83} &
  \multicolumn{2}{c}{27.01} &
  \multicolumn{2}{c}{7.71} &
  \multicolumn{2}{c}{33.95} &
  \multicolumn{2}{c}{2.25} &
  \multicolumn{2}{c}{\underline{4.09}} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{7.95} &
  \multicolumn{2}{c}{9.20} &
  \multicolumn{2}{c}{4.81} \\
 % \multicolumn{1}{l|}{MonoOcc-S~\cite{zheng2024monoocc}} &
 % \multicolumn{1}{c|}{S}&
 %  - &
 %  \multicolumn{1}{c|}{13.80} &
 %  \multicolumn{2}{c}{55.20} &
 %  \multicolumn{2}{c}{27.80} &
 %  \multicolumn{2}{c}{25.10} &
 %  \multicolumn{2}{c}{9.70} &
 %  \multicolumn{2}{c}{21.40} &
 %  \multicolumn{2}{c}{23.20} &
 %  \multicolumn{2}{c}{5.20} &
 %  \multicolumn{2}{c}{2.20} &
 %  \multicolumn{2}{c}{1.50} &
 %  \multicolumn{2}{c}{5.40} &
 %  \multicolumn{2}{c}{24.00} &
 %  \multicolumn{2}{c}{8.70} &
 %  \multicolumn{2}{c}{23.00} &
 %  \multicolumn{2}{c}{1.70} &
 %  \multicolumn{2}{c}{2.00} &
 %  \multicolumn{2}{c}{0.20} &
 %  \multicolumn{2}{c}{13.40} &
 %  \multicolumn{2}{c}{5.80} &
 %  \multicolumn{2}{c}{6.40} \\
 
 % \multicolumn{1}{l|}{H2GFormer-S~\cite{wang2024h2gformer}} &
 % \multicolumn{1}{c|}{S}&
 %  44.20 &
 %  \multicolumn{1}{c|}{13.72} &
 %  \multicolumn{2}{c}{56.40} &
 %  \multicolumn{2}{c}{28.60} &
 %  \multicolumn{2}{c}{26.50} &
 %  \multicolumn{2}{c}{4.90} &
 %  \multicolumn{2}{c}{22.80} &
 %  \multicolumn{2}{c}{23.40} &
 %  \multicolumn{2}{c}{4.80} &
 %  \multicolumn{2}{c}{0.80} &
 %  \multicolumn{2}{c}{0.90} &
 %  \multicolumn{2}{c}{4.10} &
 %  \multicolumn{2}{c}{24.60} &
 %  \multicolumn{2}{c}{9.10} &
 %  \multicolumn{2}{c}{23.80} &
 %  \multicolumn{2}{c}{1.20} &
 %  \multicolumn{2}{c}{2.50} &
 %  \multicolumn{2}{c}{0.10} &
 %  \multicolumn{2}{c}{13.30} &
 %  \multicolumn{2}{c}{6.40} &
 %  \multicolumn{2}{c}{6.30} \\
 \multicolumn{1}{l|}{H2GFormer-T~\cite{wang2024h2gformer}} &
 \multicolumn{1}{c|}{S-T}&
  44.69 &
  \multicolumn{1}{c|}{14.29} &
  \multicolumn{2}{c}{57.00} &
  \multicolumn{2}{c}{29.37} &
  \multicolumn{2}{c}{21.74} &
  \multicolumn{2}{c}{0.34} &
  \multicolumn{2}{c}{20.51} &
  \multicolumn{2}{c}{28.21} &
  \multicolumn{2}{c}{6.80} &
  \multicolumn{2}{c}{0.95} &
  \multicolumn{2}{c}{0.91} &
  \multicolumn{2}{c}{9.32} &
  \multicolumn{2}{c}{\underline{27.44}} &
  \multicolumn{2}{c}{7.80} &
  \multicolumn{2}{c}{36.26} &
  \multicolumn{2}{c}{1.15} &
  \multicolumn{2}{c}{0.10} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{7.98} &
  \multicolumn{2}{c}{9.88} &
  \multicolumn{2}{c}{{{5.81}}} \\
 \multicolumn{1}{l|}{Symphonies~\cite{jiang2024symphonize}} &
 \multicolumn{1}{c|}{S}&
  41.92 &
  \multicolumn{1}{c|}{14.89} &
  \multicolumn{2}{c}{56.37} &
  \multicolumn{2}{c}{27.58} &
  \multicolumn{2}{c}{15.28} &
  \multicolumn{2}{c}{\underline{0.95}} &
  \multicolumn{2}{c}{21.64} &
  \multicolumn{2}{c}{28.68} &
  \multicolumn{2}{c}{\underline{20.44}} &
  \multicolumn{2}{c}{2.54} &
  \multicolumn{2}{c}{\textbf{{2.82}}} &
  \multicolumn{2}{c}{\textbf{13.89}} &
  \multicolumn{2}{c}{25.72} &
  \multicolumn{2}{c}{6.60} &
  \multicolumn{2}{c}{30.87} &
  \multicolumn{2}{c}{\textbf{{3.52}}} &
  \multicolumn{2}{c}{2.24} &
  \multicolumn{2}{c}{{{0.00}}} &
  \multicolumn{2}{c}{8.40} &
  \multicolumn{2}{c}{9.57} &
  \multicolumn{2}{c}{5.76} \\
 % \multicolumn{1}{l|}{StereoScene~\cite{li2024bridgingstereogeometrybev}} &
 % \multicolumn{1}{c|}{S}&
 %   &
 %  \multicolumn{1}{c|}{15.36} &
 %  \multicolumn{2}{c}{61.90} &
 %  \multicolumn{2}{c}{31.20} &
 %  \multicolumn{2}{c}{30.70} &
 %  \multicolumn{2}{c}{10.70} &
 %  \multicolumn{2}{c}{24.20} &
 %  \multicolumn{2}{c}{22.80} &
 %  \multicolumn{2}{c}{2.80} &
 %  \multicolumn{2}{c}{3.40} &
 %  \multicolumn{2}{c}{2.40} &
 %  \multicolumn{2}{c}{\underline{{6.10}}} &
 %  \multicolumn{2}{c}{23.80} &
 %  \multicolumn{2}{c}{8.40} &
 %  \multicolumn{2}{c}{27.00} &
 %  \multicolumn{2}{c}{\underline{{2.90}}} &
 %  \multicolumn{2}{c}{2.20} &
 %  \multicolumn{2}{c}{0.50} &
 %  \multicolumn{2}{c}{16.50} &
 %  \multicolumn{2}{c}{7.00} &
 %  \multicolumn{2}{c}{7.20} \\
% \multicolumn{1}{l|}{MonoOcc-L~\cite{zheng2024monoocc}} &
%  \multicolumn{1}{c|}{S}&
%    &
%   \multicolumn{1}{c|}{15.63} &
%   \multicolumn{2}{c}{59.10} &
%   \multicolumn{2}{c}{30.90} &
%   \multicolumn{2}{c}{27.10} &
%   \multicolumn{2}{c}{9.80} &
%   \multicolumn{2}{c}{22.90} &
%   \multicolumn{2}{c}{23.90} &
%   \multicolumn{2}{c}{\underline{{7.20}}} &
%   \multicolumn{2}{c}{\textbf{{4.50}}} &
%   \multicolumn{2}{c}{2.40} &
%   \multicolumn{2}{c}{\textbf{{7.70}}} &
%   \multicolumn{2}{c}{25.00} &
%   \multicolumn{2}{c}{9.80} &
%   \multicolumn{2}{c}{26.10} &
%   \multicolumn{2}{c}{2.80} &
%   \multicolumn{2}{c}{\underline{{4.70}}} &
%   \multicolumn{2}{c}{0.60} &
%   \multicolumn{2}{c}{16.90} &
%   \multicolumn{2}{c}{7.30} &
%   \multicolumn{2}{c}{8.40} \\
 \multicolumn{1}{l|}{CGFormer~\cite{yu2024contextgeometryawarevoxel}} &
 \multicolumn{1}{c|}{S}&
  \textbf{{45.99}} &
  \multicolumn{1}{c|}{16.87} &
  \multicolumn{2}{c}{\underline{65.51}} &
  \multicolumn{2}{c}{32.31} &
  \multicolumn{2}{c}{{{20.82}}} &
  \multicolumn{2}{c}{0.16} &
  \multicolumn{2}{c}{\underline{{23.52}}} &
  \multicolumn{2}{c}{\textbf{34.32}} &
  \multicolumn{2}{c}{19.44} &
  \multicolumn{2}{c}{\textbf{{4.61}}} &
  \multicolumn{2}{c}{2.71} &
  \multicolumn{2}{c}{7.67} &
  \multicolumn{2}{c}{26.93} &
  \multicolumn{2}{c}{\textbf{{8.83}}} &
  \multicolumn{2}{c}{\textbf{39.54}} &
  \multicolumn{2}{c}{2.38} &
  \multicolumn{2}{c}{4.08} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{9.20} &
  \multicolumn{2}{c}{\underline{{10.67}}} &
  \multicolumn{2}{c}{\textbf{{7.84}}} \\
% Bi-SSC~\cite{Xue_2024_CVPR} &
%   \textbf{{45.10}} &
%   \multicolumn{1}{c|}{16.73} &
%   \multicolumn{2}{c}{63.40} &
%   \multicolumn{2}{c}{33.30} &
%   \multicolumn{2}{c}{31.70} &
%   \multicolumn{2}{c}{11.20} &
%   \multicolumn{2}{c}{\textbf{{26.60}}} &
%   \multicolumn{2}{c}{25.00} &
%   \multicolumn{2}{c}{6.80} &
%   \multicolumn{2}{c}{1.80} &
%   \multicolumn{2}{c}{1.00} &
%   \multicolumn{2}{c}{\underline{{6.80}}} &
%   \multicolumn{2}{c}{\textbf{{26.10}}} &
%   \multicolumn{2}{c}{10.50} &
%   \multicolumn{2}{c}{28.90} &
%   \multicolumn{2}{c}{1.70} &
%   \multicolumn{2}{c}{3.30} &
%   \multicolumn{2}{c}{\underline{{1.00}}} &
%   \multicolumn{2}{c}{19.40} &
%   \multicolumn{2}{c}{\textbf{{9.30}}} &
%   \multicolumn{2}{c}{8.40} \\
\multicolumn{1}{l|}{HTCL-S~\cite{li2024hierarchical}} &
\multicolumn{1}{c|}{S-T}&
  {{45.51}} &
  \multicolumn{1}{c|}{\textbf{{17.13}}} &
  \multicolumn{2}{c}{{63.70}} &
  \multicolumn{2}{c}{\underline{{32.48}}} &
  \multicolumn{2}{c}{\underline{{23.27}}} &
  \multicolumn{2}{c}{{0.14}} &
  \multicolumn{2}{c}{\textbf{24.13}} &
  \multicolumn{2}{c}{\underline{{34.30}}} &
  \multicolumn{2}{c}{\textbf{20.72}} &
  \multicolumn{2}{c}{\underline{3.99}} &
  \multicolumn{2}{c}{\underline{{2.80}}} &
  \multicolumn{2}{c}{\underline{{11.99}}} &
  \multicolumn{2}{c}{{{26.96}}} &
  \multicolumn{2}{c}{\underline{{8.79}}} &
  \multicolumn{2}{c}{{{37.73}}} &
  \multicolumn{2}{c}{2.56} &
  \multicolumn{2}{c}{{{2.30}}} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{\textbf{{11.22}}} &
  \multicolumn{2}{c}{\textbf{11.49}} &
  \multicolumn{2}{c}{{{6.95}}} \\ 

  
 \rowcolor{violet!7}\multicolumn{1}{l|}{\textbf{ScanSSC (ours)}}&
 \multicolumn{1}{c|}{S}&
 \underline{45.95} &
  \multicolumn{1}{c|}{\underline{{17.12}}} &
  \multicolumn{2}{c}{\textbf{{66.70}}} &
  \multicolumn{2}{c}{\textbf{{33.87}}} &
  \multicolumn{2}{c}{\textbf{{24.75}}} &
  \multicolumn{2}{c}{{0.20}} &
  \multicolumn{2}{c}{22.42} &
  \multicolumn{2}{c}{{{34.16}}} &
  \multicolumn{2}{c}{14.78} &
  \multicolumn{2}{c}{3.81} &
  \multicolumn{2}{c}{{2.19}} &
  \multicolumn{2}{c}{{{9.81}}} &
  \multicolumn{2}{c}{\textbf{{27.59}}} &
  \multicolumn{2}{c}{{{8.31}}} &
  \multicolumn{2}{c}{\underline{{39.26}}} &
  \multicolumn{2}{c}{\underline{2.87}} &
  \multicolumn{2}{c}{\textbf{{5.93}}} &
  \multicolumn{2}{c}{0.00} &
  \multicolumn{2}{c}{\underline{{10.52}}} &
  \multicolumn{2}{c}{10.52} &
  \multicolumn{2}{c}{\underline{{7.50}}} \\ \hline
\end{tabular}%
}
\vspace{-0.2cm}
\caption{Quantitative results on SemanticKITTI hidden test set. `M', `S', and `S-T' represent the monocular, stereo, and temporal stereo inputs, respectively. \textbf{Bold} and \underline{underline} highlight the best and second-best results, respectively.}
\vspace{-0.2cm}
% {Red} and \textcolor{blue}{blue} highlight the best and second-best results, respectively.}
\label{tab:SemKITTI_valid}
    
\end{table*}

